Capabilities and Skills in Manufacturing: A Survey Over the Last Decade of ETFA

Industry 4.0 envisions Cyber-Physical Production Systems (CPPSs) to foster adaptive production of mass-customizable products. Manufacturing approaches based on capabilities and skills aim to support this adaptability by encapsulating machine functions and decoupling them from specific production processes. At the 2022 IEEE conference on Emerging Technologies and Factory Automation (ETFA), a special session on capability- and skill-based manufacturing is hosted for the fourth time. However, an overview on capability- and skill based systems in factory automation and manufacturing systems is missing. This paper aims to provide such an overview and give insights to this particular field of research. We conducted a concise literature survey of papers covering the topics of capabilities and skills in manufacturing from the last ten years of the ETFA conference. We found 247 papers with a notion on capabilities and skills and identified and analyzed 34 relevant papers which met this survey's inclusion criteria. In this paper, we provide (i) an overview of the research field, (ii) an analysis of the characteristics of capabilities and skills, and (iii) a discussion on gaps and opportunities.

==> Fundamentals.tex <==
%Findings zu den Grundlagen (z.B. Definitionen, …).
%Gegenüberstellung von Grundlagen aus der Literatur mit Grundlagen-Fragen des Fragebogens

==> barchart.tex <==
\begin{tikzpicture}
    \footnotesize
    \begin{axis}[
        xbar,
        xmin = -.25,
        axis lines* = middle,
        ymajorticks = false,
        every inner y axis line/.append style = {dashed},
        nodes near coords,
        nodes near coords style = {anchor = west},
        point meta = explicit symbolic,
        xtick = {0,2,4,...,14},
        ytick = {0,2,...,38},
        bar width=0.25cm,
        % y = 0.3cm,
        ]
        \addplot [fill=blue!30,draw=none] coordinates {
(13,35)[fortiss GmbH]
(5,34)[Festo SE \& Co. KG]
(4,33)[Otto von Guericke University Magdeburg]
(3,32)[Fraunhofer IGCV]
(3,31)[Helmut Schmidt University]
(3,30)[Johannes Kepler University]
(3,29)[RWTH Aachen University]
(3,28)[Technical University of Munich]
(3,27)[TU Wien]
(3,26)[Volkswagen AG]
(2,25)[Fraunhofer IOSB]
(2,24)[KUKA Deutschland GmbH]
(2,23)[Loughborough University]
(2,22)[ProFactor GmbH]
(2,21)[Siemens AG]
(2,20)[University of Applied Sciences Upper Austria]
(1,19)[ABB Corporate Research Center]
(1,18)[Autonomous Intelligent Driving GmbH]
(1,17)[CAX-Service GmbH]
(1,16)[Fraunhofer IESE]
(1,15)[FZI Research Center for Information Technology]
(1,14)[German Research Center for Artificial Intelligence]
(1,13)[Introsys SA]
(1,12)[Karlsruhe Institute of Technology]
(1,11)[National Research Council of Italy]
(1,10)[OWL University of Applied Sciences and Arts]
(1,9)[Pro2Future GmbH]
(1,8)[Robert Bosch GmbH]
(1,7)[Sorbonne Université]
(1,6)[Université Paris-Saclay]
(1,5)[University of Augsburg]
(1,4)[University of Brescia]
(1,3)[University of Southern Denmark]
(1,2)[VDMA Robotics and Automation Association]
(1,1)[WEISS GmbH]
        };
    \end{axis}
\end{tikzpicture}

\begin{tikzpicture}
\scriptsize
\begin{axis} [
    xbar,
    axis lines* = middle,
    every inner y axis line/.append style = {dashed},
    nodes near coords,
    nodes near coords style = {anchor = west},
    bar width=5pt,
    point meta = explicit symbolic,
    ymajorticks = false,
    width = \columnwidth,
    height = 12cm,
    xmax = 15,
    ymax = 40,
    ]
\addplot[fill=blue!30,draw=none] coordinates {
(13,35)[fortiss GmbH]
(5,34)[Festo SE \& Co. KG]
(4,33)[Otto von Guericke University Magdeburg]
(3,32)[Fraunhofer IGCV]
(3,31)[Helmut Schmidt University]
(3,30)[Johannes Kepler University]
(3,29)[RWTH Aachen University]
(3,28)[Technical University of Munich]
(3,27)[TU Wien]
(3,26)[Volkswagen AG]
(2,25)[Fraunhofer IOSB]
(2,24)[KUKA Deutschland GmbH]
(2,23)[Loughborough University]
(2,22)[ProFactor GmbH]
(2,21)[Siemens AG]
(2,20)[University of Applied Sciences Upper Austria]
(1,19)[ABB Corporate Research Center]
(1,18)[Autonomous Intelligent Driving GmbH]
(1,17)[CAX-Service GmbH]
(1,16)[Fraunhofer IESE]
(1,15)[FZI Research Center for Information Technology]
(1,14)[German Research Center for Artificial Intelligence]
(1,13)[Introsys SA]
(1,12)[Karlsruhe Institute of Technology]
(1,11)[National Research Council of Italy]
(1,10)[OWL University of Applied Sciences and Arts]
(1,9)[Pro2Future GmbH]
(1,8)[Robert Bosch GmbH]
(1,7)[Sorbonne Université]
(1,6)[Université Paris-Saclay]
(1,5)[University of Augsburg]
(1,4)[University of Brescia]
(1,3)[University of Southern Denmark]
(1,2)[VDMA Robotics and Automation Association]
(1,1)[WEISS GmbH]
};
\end{axis}
 
\end{tikzpicture}
